Watch Your Language: Investigating Content Moderation with Large Language Models

Large language models (LLMs) have exploded in popularity due to their ability to perform a wide array of natural language tasks. Text-based content moderation is one LLM use case that has received recent enthusiasm, however, there is little research investigating how LLMs perform in content moderation settings. In this work, we evaluate a suite of commodity LLMs on two common content moderation tasks: rule-based community moderation and toxic content detection. For rule-based community moderation, we instantiate 95 subcommunity specific LLMs by prompting GPT-3.5 with rules from 95 Reddit subcommunities. We find that GPT-3.5 is effective at rule-based moderation for many communities, achieving a median accuracy of 64% and a median precision of 83%. For toxicity detection, we evaluate a suite of commodity LLMs (GPT-3, GPT-3.5, GPT-4, Gemini Pro, LLAMA 2) and show that LLMs significantly outperform currently widespread toxicity classifiers. However, recent increases in model size add only marginal benefit to toxicity detection, suggesting a potential performance plateau for LLMs on toxicity detection tasks. We conclude by outlining avenues for future work in studying LLMs and content moderation.

==> methodology.tex <==
\section{Methodology}
\label{sec:methodology}
The goal of our work is to evaluate how well state-of-the-art language models fare at two common content moderation tasks: rule-based community moderation and toxicity detection. In this section, we detail our evaluation datasets, our language model prompts, and our evaluation strategies. Our data and code will be made available at publication time.

\subsection{Rule-Based Community Moderation}
\subsubsection{Collecting ground-truth moderation decisions}
To compare how well LLMs align with human-provided moderation decisions, we leverage a dataset created by Chandrasekharan et~al.~\shortcite{chandrasekharan2018internet} that contains comments that were moderated from 100~popular subreddits between 2016--2017. Since their study was conducted, 5~subreddits have gone offline or been removed from the platform, so our study focuses on the remaining 95~subreddits. For each subreddit, we sample 500~comments that were removed by moderators as well as 500~comments that were \textit{not} removed by moderators during the same time period, thus creating a \textit{balanced dataset} of moderation decisions for each subreddit. These datasets serve as our baseline for rule-based evaluation.

\subsubsection{Extracting Subreddit metadata}
We first extract the description of each subreddit using the Reddit API. We then extract the moderation rules of that community by using the Reddit rules API\footnote{https://www.reddit.com/dev/api/\#GET\_r\_subreddit\_about\_rules}, which provides a list of rule texts and whether the rule applies to a post, comment, or all content posted to the subreddit. Given we are only investigating comment moderation in this study, we filter any rules that do not apply to comments. We extract the full rule text for each rule and build a numbered list of rules that we use to prompt each model. 
%We provide a full example of one such rule text for the subreddit \texttt{AskReddit} in the Appendix.

\subsubsection{Prompt design}
We construct a new zero-shot prompted LLM-engine for each subreddit we investigate. We begin by prompting the LLM with the description of the subreddit as well as the constructed rules string for each subcommunity. The full initial prompt text is:

\begin{small}
\begin{verbatim}
You are a helpful content moderation 
assistant for the online subreddit 
<subreddit>. The subreddit has the 
following description: <description>.

Here are the rules for the subreddit:
<rule_texts>
\end{verbatim}
\end{small}

We then ask the model to evaluate whether it would moderate new unseen comments (yes/no), the rule text and rule numbers that the comment violates, and an explanation for the decision. Similarly to the toxic content detection task, we ask the model to return a JSON object for downstream analysis. The full prompt text is:

\begin{small}
\begin{verbatim}
Consider the following comment:
<example_comment>

Return a JSON object with four fields, 
"would_moderate," that is 
either "yes" or "no" depending 
on if you would remove this comment 
from the subreddit, "rules" which are 
the text of the rules being violated, 
"rule_nums" which are a comma-separated
list of rules being violated, "rating"
which is a score from 1--5 on how 
violative the comment is.
\end{verbatim}
\end{small}
%, and "explanation" which contains 
%a reason for your decision.


\subsubsection{Evaluation strategy}
We compare ground-truth moderation decisions with decisions made by each subreddit-specific tuned LLM on a number of binary performance metrics. For this experiment, we solely rely on OpenAI's GPT3.5 for evaluation as it well balances at-scale measurements (i.e., ~100,000 queries in total) with cost. To understand \textit{why} the LLM makes mistakes, we also perform a case study on mistakes created in the \texttt{r/worldnews} subreddit and provide a qualitative analysis of existing gaps in rule-based moderation.

\subsection{Toxic content detection}

\subsubsection{Dataset}
We leverage a dataset of toxicity annotations curated by Kumar et~al.~\shortcite{kumar2021designing} that consists of 107K~comments sourced from three social platforms: Reddit, Twitter, and 4chan. Each comment was labeled for toxicity by five~raters on a 5-point Likert scale from ``not at all toxic'' to ``very toxic.'' We collapse this score into a binary outcome based on the median toxicity rating. If the median rating was equal to or above ``moderately toxic'' we denote the comment as toxic, and if the rating was below this threshold we denote the comment as non-toxic. Due to cost limitations, we do not evaluate each LLM on the entire dataset. Rather, we sample the aggregate dataset to build a balanced dataset of toxicity annotations that contains 5000~examples of toxic content and 5000~examples of nontoxic content. We will release this golden dataset at publication time.

%One challenge to consider when evaluating LLMs published by industry is that their training data is unknown to researcher a priori. In order to ensure we are testing each LLM in an out-of-distribution context, we leverage a toxic content dataset created by our research team in prior work (blinded for submission) that we release to researchers on request. Because no one from the OpenAI team reached out to us for data access, we believe the text of dataset is unlikely to be included in their training data. 

\subsubsection{Prompt design}
We first prompt each LLM with the definition of toxic content used by Google Jigsaw, which is ``a rude, disrespectful, or unreasonable comment that is likely to make someone leave a discussion'' ~\cite{perspectiveapi}. We then ask the model to rate the toxicity of unseen comments on a scale from 1--10, as well as to provide an explanation for the rating in natural language. For ease of downstream analysis, we prompted the LLM to always return results as a JSON object with consistent indexing. The full prompt text is: 

\begin{small}
\begin{verbatim}
Consider the following comment: 
<example_comment>

Return a JSON object with a two fields, 
"rating," that is a score from 1 to 5 
depending on how toxic the comment is 
based on our definition, and "explanation" 
which contains a reason for the rating.    
\end{verbatim}
\end{small}

\subsubsection{Evaluation strategy}
We evaluate three state-of-the-art LLMs for this task---OpenAI's GPT3, OpenAI's GPT3.5 (i.e., ChatGPT), and OpenAI's GPT4. We chose these as they represent recent, publicly available LLM offerings on the market and covers a range of model sizes and training strategies. To compare across a SOTA commodity baseline, we also label each comment using the Google Jigsaw Perspective API~\cite{perspectiveapi} using their \texttt{TOXICITY} and \texttt{SEVERE\_TOXICITY} classifiers at varying thresholds.



\subsection{Limitations}
This work primarily focuses on text-based content moderation tasks, and specifically on comment moderation on discussion oriented platforms. As such, our results may not extend to other types of moderation, for example, those involving mixed modalities (i.e., images, videos, etc.) or those on social platforms with other affordances (i.e., real-time communication). Furthermore, our evaluation here is done on \textit{balanced datasets} and thus our comment distributions do not reflect comment distributions found in real-world platforms. We also note that while our results are promising, the LLMs we tested are currently \textit{too expensive} to immediately impact most content moderation contexts, and future research is needed to build models that can balance performance with cost.
